Non-polynomial Worst-Case Analysis of Recursive Programs

We study the problem of developing efficient approaches for proving worst-case bounds of non-deterministic recursive programs. Ranking functions are sound and complete for proving termination and worst-case bounds of nonrecursive programs. First, we apply ranking functions to recursion, resulting in measure functions. We show that measure functions provide a sound and complete approach to prove worst-case bounds of non-deterministic recursive programs. Our second contribution is the synthesis of measure functions in nonpolynomial forms. We show that non-polynomial measure functions with logarithm and exponentiation can be synthesized through abstraction of logarithmic or exponentiation terms, Farkas' Lemma, and Handelman's Theorem using linear programming. While previous methods obtain worst-case polynomial bounds, our approach can synthesize bounds of the form $\mathcal{O}(n\log n)$ as well as $\mathcal{O}(n^r)$ where $r$ is not an integer. We present experimental results to demonstrate that our approach can obtain efficiently worst-case bounds of classical recursive algorithms such as (i) Merge-Sort, the divide-and-conquer algorithm for the Closest-Pair problem, where we obtain $\mathcal{O}(n \log n)$ worst-case bound, and (ii) Karatsuba's algorithm for polynomial multiplication and Strassen's algorithm for matrix multiplication, where we obtain $\mathcal{O}(n^r)$ bound such that $r$ is not an integer and close to the best-known bounds for the respective algorithms.

==> input_spec.tex <==
Concretely, the user needs to provide the following items as input to our tool for each of the examples:
\begin{itemize}
	\item An implementation of the programs as illustrated in Figures \ref{fig:mergesort, fig:karatsubaa, fig:karatsubab, fig:closestpaira, fig:closestpairb, fig:closestpairc, fig:closestpaird, fig:strassena, fig:strassenb, fig:strassenc}. 
	\item Invariants at significant labels (cut-points). These can be straightforwardly calculated from the branching conditions and there are also tools to infer such invariants, such as \cite{DBLP:conf/cav/ColonSS03, DBLP:conf/popl/CousotC77}.
	\item The type of bound to be synthesized, i.e. $\mathrm{op}$. For Merge-Sort and Closest-Pair, the user should choose to obtain a logarithmic bound and for Strassen's and Karatsuba's algorithms, a bound of the form $O(n^r)$.
	\begin{itemize}
		\item In the latter case, the user should specify an upper-bound on $r$.
	\end{itemize}
	\item Maximum number, $d$, of terms in any multiplicand of the summand in equation \ref{eq:synform}. For all of our examples, $d$ can be set to $2$.  
\end{itemize}


Furthermore, once the user-specified maximum degree, $d$, for the template is fixed, 
then the complexity of our algorithm is polynomial. 
While our algorithm is exponential in $d$, in all our examples the maximum degree is 2. Note that $d$ is the number of terms multiplied together in each summand of the general form as in (\ref{eq:synform}). For example,
(i) for $n^{4.5} $ there is only one term, and hence $d=1$;
(ii) for $n^{3.9} \cdot \log n$  we have two terms, and hence $d=2$.
Therefore, even for worst-case non-polynomial bounds of higher degrees, the maximum degree for template is still small.


==> termination.tex <==


\vspace{-1.5em}
\section{Termination over Non-deterministic Recursive Programs}\label{sect:termination}
\vspace{-0.8em}
In this section, we describe the notion of termination time for
nondeterministic
recursive programs and the problem we study.
Below we fix a nondeterministic
recursive program $W$ and its CFG taking the form ($\dag$).

In this paper, we study the problem of automatically deriving upper bounds for
$\overline{T}(\centerdot)$.
A very useful notion to achieve this is an \emph{invariant} for the input
recursive program, where an invariant specifies logical formulae
which all ``reachable'' stack elements must satisfy.
Below we define reachable stack elements and invariants.

%%\smallskip
\begin{definition}[Reachability]\label{def:reachability}
Let $\fn{f}^*$ be a function name and $\phi^*$ be a propositional arithmetic predicate over $\pvars{f^*}$.
A configuration $w$ is \emph{reachable} w.r.t $\fn{f}^*,\phi^*$ if there exist a scheduler $\pi$ and a non-terminal stack element $(\fn{f}^*,\lin{\fn{f}^*},\nu)$ such that (i) $\nu\models\phi^*$ and (ii)
$w$ appears in the run $\rho((\fn{f}^*,\lin{\fn{f}^*},\nu),\pi)$.
A stack element $\mathfrak{c}$ is \emph{reachable} w.r.t $\fn{f}^*,\phi^*$
if there exists a configuration $w$ reachable w.r.t $\fn{f}^*,\phi^*$ such that $w=\mathfrak{c}\cdot w'$ for some configuration $w'$.
\end{definition}

%%\smallskip
\begin{definition}[Invariants]\label{def:inv}
A (linear) \emph{invariant} $\inv$ w.r.t a function name $\fn{f}^*$ and a propositional
arithmetic predicate $\phi^*$ over $\pvars{f^*}$ is a function that upon
any pair $(\fn{f},\loc)$ satisfying $\fn{f}\in\fnames$ and
$\loc\in\locs{f}\backslash\{\lout{\fn{f}}\}$, $I(\fn{f},\loc)$ is a propositional arithmetic predicate
over $\pvars{f}$
such that (i) $I(\fn{f},\loc)$ is without the appearance of floored expressions (i.e. $\lfloor\centerdot\rfloor$) and (ii) for all stack elements $(\fn{f},\loc,\nu)$ reachable w.r.t
$\fn{f}^*,\phi^*$, $\nu\models I(\fn{f},\loc)$.
$I$ is in \emph{disjunctive normal form} if every $I(\fn{f},\loc)$ is in disjunctive normal form.
\end{definition}

In the algorithmic problem we study (cf. below), we assume that an invariant is given as input;
moreover, we omit the role of $\fn{f}^*,\phi^*$ and integrate it into the input invariant.
Although requiring an input invariant seems to make our algorithm less applicable,
there exist many ways to derive linear invariants automatically (e.g., through abstract interpretation~\cite{DBLP:conf/popl/CousotC77} or Farkas' Lemma~\cite{DBLP:conf/cav/ColonSS03}).
Moreover, all concrete invariants used in this paper can be inferred directly from the initial arithmetic predicate $\phi^*$ and the guards of if-branches and while-loops.

\smallskip\noindent{\bf The \recterm\ problem.}
In this work we consider the algorithmic problem of automatically deriving upper bounds
for termination time of recursive programs, which we refer to as the \recterm\
problem, formally, defined as follows:
\begin{compactitem}
\item \emph{Input:} a recursive program $W$, an invariant $\inv$ in disjunctive normal form and a quadruple $(d, \mathrm{op}, r,k)$ of parameters where $d\in\Nset$ is the degree of the measure function to be synthesized, $\mathrm{op}\in\{\mathrm{log}, \mathrm{exp}\}$ signals either logarithmic (when $\mathrm{op}=\log$) (e.g., $n\ln{n}$) or exponential (when $\mathrm{op}=\mathrm{exp}$) (e.g., $n^{1.6}$) measure functions, $r$ is a rational number greater than $1$ which specifies the exponent in the measure function (i.e., $n^r$) when $\mathrm{op}=\mathrm{exp}$ and $k\in\Nset$ is a parameter to our algorithm;
\item \emph{Output:} a function $h$ from the set of stack elements into $[0,\infty]$ (in a form determined by $(d, \mathrm{op}, r)$ to be specified later)
such that $\overline{T}(\fn{f}, \loc, \nu)\le h(\nu)$ whenever $\nu\in\Aval{f}$ and $\nu\models I(\fn{f},\loc)$.
\end{compactitem}
Note that although in the input we fix the exponent $r$ when $\mathrm{op}=\mathrm{exp}$, one can iterate our algorithm through binary search over an input bounded range so as to obtain a measure function falling in the given range as precise as possible.

